On the Approximation of Accuracy-configurable Sequential Multipliers via Segmented Carry Chains

In this paper, we present a multiplier based on a sequence of approximated accumulations. According to a given splitting point of the carry chains, the technique herein introduced allows varying the quality of the accumulations and, consequently, the overall product. Our approximate multiplier trades-off accuracy for a reduced latency (with respect to an accurate sequential multiplier) and exploits the inherent area savings of sequential over combinatorial approaches. We implemented multiple versions with different bit-width and accuracy configurations, targeting an FPGA and a 45nm ASIC to estimate resources, power consumption, and latency. We also present two error analyses of the proposed design based on closed-form analysis and simulations.

==> tables/asic_measurements.tex <==
\newcommand{\wc}[1]{\color{white}\textbf{#1}}
\newcommand{\mrc}[1]{\multicolumn{1}{c}{\multirow{-2}{*}{\wc{#1}}}}
\newcommand{\cmc}[1]{\multicolumn{2}{c}{\multirow{-2}{*}{\wc{#1}}}}
\newcommand{\ccw}{\cellcolor{white}}
\newcommand{\rca}{\rowcolor{aliceblue!75}}
\newcommand{\rcb}{\rowcolor{blue_fau!75}}
\setlength\arrayrulewidth{0.8pt}
\small
\sisetup{table-format          = 5.2,
         group-separator       = {,},
         output-decimal-marker = {.},
         group-four-digits
        }
\begin{tabular}{lrrS[table-format=1.3]S[table-format=6.3]S[table-format=3.3]}
    \hline
    \rcb
                       &                  &   &                      &                        &                    \\
    \rcb
    \mrc{Design}       & \cmc{Bitwidth $(n)$} & \mrc{Latency $[ns]$} & \mrc{Area $[\mu m^2]$} & \mrc{Power $[mW]$} \\
    \hline
    \rca
    \ccw               & $4{\times}4$     &   & 0.425                & 135.66                 & 0.025              \\
                       & $8{\times}8$     &   & 1.227                & 427.728                & 0.119              \\
    \rca
    \ccw Combinatorial & $16{\times}16$   &   & 1.337                & 1424.696               & 0.883              \\
    Accurate           & $32{\times}32$   &   & 1.722                & 4731.342               & 3.784              \\
    \rca
    \ccw Multiplier    & $64{\times}64$   &   & 2.164                & 17100.076              & 15.15              \\
                       & $128{\times}128$ &   & 2.488                & 67960.34               & 62.824             \\
    \rca
    \ccw               & $256{\times}256$ &   & 2.554                & 313430.992             & 374.387            \\
    \hline
                       & $4{\times}4$     &   & 0.336                & 251.104                & 0.036              \\
    \rca
    \ccw               & $8{\times}8$     &   & 0.618                & 459.116                & 0.065              \\
    Sequential         & $16{\times}16$   &   & 0.788                & 901.474                & 0.174              \\
    \rca
    \ccw Accurate      & $32{\times}32$   &   & 0.846                & 1825.558               & 0.34               \\
    Multiplier         & $64{\times}64$   &   & 0.954                & 3646.062               & 0.819              \\
    \rca                    
    \ccw               & $128{\times}128$ &   & 0.982                & 7284.41                & 1.71               \\
                       & $256{\times}256$ &   & 1.112                & 14554.988              & 3.486              \\
    \hline
    \rca
    \ccw               & $4{\times}4$     &   & 0.263                & 267.064                & 0.038              \\
                       & $8{\times}8$     &   & 0.407                & 479.864                & 0.064              \\
    \rca
    \ccw Sequential    & $16{\times}16$   &   & 0.698                & 911.848                & 0.128              \\
    Approximate        & $32{\times}32$   &   & 0.823                & 1845.242               & 0.36               \\
    \rca
    \ccw Multiplier    & $64{\times}64$   &   & 0.856                & 3707.242               & 0.785              \\
    $t=\frac{n}{2}$    & $128{\times}128$ &   & 0.879                & 7424.592               & 1.669              \\
    \rca
    \ccw               & $256{\times}256$ &   & 0.923                & 14871.262              & 3.398              \\
    \hline
\end{tabular}


==> tables/fpga_measurements.tex <==
\newcommand{\wc}[1]{\color{white}\textbf{#1}}
\newcommand{\mrm}[1]{\multicolumn{1}{c}{\multirow{-2}{*}{\wc{#1}}}}
\newcommand{\mrc}[1]{\multicolumn{1}{c}{\wc{#1}}}
\newcommand{\cmc}[1]{\multicolumn{2}{c}{\wc{#1}}}
\newcommand{\ccw}{\cellcolor{white}}
\newcommand{\rca}{\rowcolor{aliceblue!75}}
\newcommand{\rcb}{\rowcolor{blue_fau!75}}
\setlength\arrayrulewidth{0.8pt}
\small
\begin{tabular}{lrrS[table-format=2.2]S[table-format=5.0]S[table-format=4.0]S[table-format=4.0]S[table-format=3.0]}
    \hline
    \rcb
                        & \cmc{Bitwidth}   & \mrc{Latency} &            &              &           & \mrc{Power}    \\
    \rcb
    \mrm{Design}        & \cmc{$(n)$}      & \mrc{$[ns]$}  & \mrm{LUTs} & \mrm{Carry4} & \mrm{FFs} & \mrc{$[mW]$}   \\
    \hline
    \rca
    \ccw                & $4{\times}4$     &   & 2.79      & 17         & 2            & 0         & 4 \\
                        & $8{\times}8$     &   & 4.71      & 72         & 10           & 0         & 5 \\
    \rca
    \ccw Combinatorial  & $16{\times}16$   &   & 6.19      & 294        & 40           & 0         & 7 \\
    Accurate            & $32{\times}32$   &   & 8.03      & 1086       & 144          & 0         & 10 \\
    \rca
    \ccw Multiplier     & $64{\times}64$   &   & 10.24     & 4390       & 577          & 0         & 20 \\
                        & $128{\times}128$ &   & 12.66     & 17432      & 2164         & 0         & 46 \\
    \rca
    \ccw                & $256{\times}256$ &   & 16.56     & 71090      & 8518         & 0         & 125 \\
    \hline
                        & $4{\times}4$     &   & 1.35      & 27         & 0            & 24        & 3 \\
    \rca
    \ccw                & $8{\times}8$     &   & 1.46      & 46         & 2            & 41        & 4 \\
    Sequential          & $16{\times}16$   &   & 1.58      & 83         & 4            & 74        & 6 \\
    \rca
    \ccw Accurate       & $32{\times}32$   &   & 1.73      & 220        & 8            & 139       & 8 \\
    Multiplier          & $64{\times}64$   &   & 2.05      & 303        & 16           & 268       & 12 \\
    \rca                    
    \ccw                & $128{\times}128$ &   & 3.35      & 522        & 32           & 525       & 18 \\
                        & $256{\times}256$ &   & 5.11      & 906        & 64           & 1038      & 30 \\
    \hline
    \rca
    \ccw                & $4{\times}4$     &   & 1.05      & 33         & 0            & 25        & 3 \\
                        & $8{\times}8$     &   & 1.13      & 55         & 0            & 42        & 4 \\
    \rca
    \ccw  Sequential    & $16{\times}16$   &   & 1.47      & 92         & 4            & 75        & 6 \\
    Approximate         & $32{\times}32$   &   & 1.59      & 238        & 8            & 140       & 8 \\
    \rca
    \ccw Multiplier     & $64{\times}64$   &   & 1.57      & 336        & 16           & 269       & 12 \\
    $t=\frac{n}{2}$     & $128{\times}128$ &   & 2.62      & 517        & 33           & 526       & 19 \\
    \rca
    \ccw                & $256{\times}256$ &   & 3.63      & 1025       & 65           & 1040      & 36 \\
    \hline
\end{tabular}

